Modeling sRGB Camera Noise with Normalizing Flows

Noise modeling and reduction are fundamental tasks in low-level computer vision. They are particularly important for smartphone cameras relying on small sensors that exhibit visually noticeable noise. There has recently been renewed interest in using data-driven approaches to improve camera noise models via neural networks. These data-driven approaches target noise present in the raw-sensor image before it has been processed by the camera's image signal processor (ISP). Modeling noise in the RAW-rgb domain is useful for improving and testing the in-camera denoising algorithm; however, there are situations where the camera's ISP does not apply denoising or additional denoising is desired when the RAW-rgb domain image is no longer available. In such cases, the sensor noise propagates through the ISP to the final rendered image encoded in standard RGB (sRGB). The nonlinear steps on the ISP culminate in a significantly more complex noise distribution in the sRGB domain and existing raw-domain noise models are unable to capture the sRGB noise distribution. We propose a new sRGB-domain noise model based on normalizing flows that is capable of learning the complex noise distribution found in sRGB images under various ISO levels. Our normalizing flows-based approach outperforms other models by a large margin in noise modeling and synthesis tasks. We also show that image denoisers trained on noisy images synthesized with our noise model outperforms those trained with noise from baselines models.

==> figs_tables/table_ablation_denoising.tex <==
\begin{table}[t]
\centering
\begin{tabular}{ c c c }
    \hline
    Flow blocks & PSNR & SSIM \\
    \hline
    CL & 33.34 & 0.867  \\
    CCS\textsubscript{ISO only}x2 &  30.08 & 0.791 \\
    CCS\textsubscript{camera only}x2 &  29.92 & 0.746  \\
    CCS\textsubscript{clean image only}x2 &  31.17 & 0.758  \\
    CCSx2 &  32.79 & 0.872  \\
    CL-CCSx2 &  32.32 & 0.868  \\
    (CL-CCSx2)\,x2 & 33.08 & 0.896  \\
    \hline
    (CL-CCSx2)\,x4 &  34.74 & 0.912  \\
     \hline
\end{tabular}
\caption{Denoising performance of various architectures}
\label{tab:denoising_ablation_studies}
\vspace{-6mm}
\end{table}


==> figs_tables/table_num_params.tex <==
\begin{table}[h]
\centering
\begin{adjustbox}{width=\columnwidth,center}
\begin{tabular}{ c c c c c }
    \hline
    Model & $NLL$ & $D_{KL}$ & $\# Params$ \\
    \hline
     Isotropic Gaussian & 3.703 & 0.091 & 50 \\  
     Diagonal Gaussian & 3.678 & 0.079 & 150 \\ 
     Full Gaussian & 3.608 & 0.085 & 525 \\
     Heteroscedastic (NLF) & 3.642 & 0.08 & 72 & \\
     Noise Flow~[2] & 3.311 & 0.198 & 2330 & \\
     Noise Flow-Large & 3.288 & 0.227 & 6618 \\
     Our model & \textbf{3.072} & \textbf{0.044} & 6310 \\
     \hline
\end{tabular}
\end{adjustbox}
\caption{An extension to Table 1 in the paper including parameter counts for all considered noise models and an additional, larger scale Noise Flow architecture.
% Noise Flow-Large is a new experiment designed to show increasing the size of the model does not increase the performance much. We need to have model architecture designed for sRGB images.
}
\label{tab:num_params}
\vspace{-4mm}
\end{table}

==> figs_tables/table_psnr_ssim.tex <==

\begin{table}[ht]
\begin{adjustbox}{width=\columnwidth,center}
\begin{tabular}{ c c c}
    \hline
    Model & $PSNR$ & $SSIM$ \\
    \hline
     Additive White Gaussian Noise & 32.04  & 0.839\\  
     Additive Diagonal Covariance Gaussian & 32.90 & 0.854 \\ 
     Additive Full covariance Gaussian & 33.12 & 0.877\\
     Heteroscedastic Gaussian & 32.14 & 0.829 \\
     Noise Flow & 33.56 &  0.900 \\
     C2N* & 33.76 & 0.901\\
     \hline 
     Our model & \textbf{34.87} & \textbf{0.912} \\
    \hdashline
     DnCNN-Real & 36.65 & 0.922 \\
     \hline
\end{tabular}
\end{adjustbox}
\caption{Models are evaluated on the SIDD Validation set. DnCNN trained on samples from \modelname achieves better performance compared to training on synthetic
noise from baselines. 
* Their code was not available at the time of submission. The results are from their paper.}
\label{tab:psnr_ssim}
\end{table}
